On Logics and Homomorphism Closure

Predicate logic is the premier choice for specifying classes of relational structures. Homomorphisms are key to describing correspondences between relational structures. Questions concerning the interdependencies between these two means of characterizing (classes of) structures are of fundamental interest and can be highly non-trivial to answer. We investigate several problems regarding the homomorphism closure (homclosure) of the class of all (finite or arbitrary) models of logical sentences: membership of structures in a sentence's homclosure; sentence homclosedness; homclosure characterizability in a logic; normal forms for homclosed sentences in certain logics. For a wide variety of fragments of first- and second-order predicate logic, we clarify these problems' computational properties.

==> My-intro.tex <==
An important preservation theorem from model theory is the
\emph{homomorphism preservation theorem} which asserts that a first-order sentence $\phi$ is equivalent to an existential positive sentence if and only if the class of all models of $\phi$ is preserved by homomorphisms. Existential positive sentences are studied in theoretical computer science and in particular in database theory, where they are called \emph{unions of conjunctive queries} and belong to some of the most frequently encountered database queries in practice. Classes of finite structures that are closed under homomorphisms also appear naturally in theoretical computer science; for example the complement of a constraint satisfaction problem, viewed as a class of finite structures, is closed under homomorphisms. 

Rossmann showed that that the homomorphism preservation theorem also holds if we consider homomorphisms between \emph{finite} models only. The homomorphism preservation theorem also extends to some more expressive logics: for example, Feder and Vardi (2001) proved that a Datalog$(\neg)$ program,
i.e., a Datalog program where additionally atomic negation is allowed, is equivalent to a Datalog program if and only if the class of structures defined by the program is preserved by homomorphisms; in this case it is easy to see by a compactness argument that preservation under homomorphisms for all models and for all finite models is equivalent. 


Here we will be investigate the following four types of questions:
\begin{itemize}
\item Given a sentence $\phi$ from some logic and a finite structure $\mathfrak{A}$, 
decide whether $\mathfrak{A}$ belongs the the closure of the models of $\phi$ under homomorphism. 
How difficult is this problem computationally? 
We are interested in the combined complexity (where both $\mathfrak{A}$ and $\phi$ are given) 
and in the complexity where $\mathfrak{A}$ is given and $\phi$ is fixed. 
\item Given a sentence $\phi$ from some logic, decide whether the class of models of $\phi$ is closed under homomorphisms. How difficult is this problem computationally? 
\item Given a sentence $\phi$ from some logic, 
can we compute a sentence $\psi$ (either from the same logic or from a different logic) such that
the model class of $\psi$ is precisely the homomorphism closure of the model class of $\phi$? 
\item For which logics 
is there a \emph{`syntactic normal form'} such that a sentence from that logic is equivalent to a sentence in normal form if and only if the model class is closed under homomorphisms? Of course the normal form should be effectively decidable (preferably even in polynomial time). 
\end{itemize}

If the satisfiability problem for the logic under consideration is undecidable, as for example for first-order logic, we obtain that the computational problem from question one is undecidable, too. 
However, we show that the problem is decidable in 2ExpTime for the guarded negation fragment of first-order logic, and in fact complete for this complexity class. 
We also prove decidability and complexity completeness results for the triguarded fragment, the two-variable fragment, and various quantifier prefix classes of first-order logic (Theorem~\ref{thm:first-main}). Each of the results holds both in the setting where we consider arbitrary models \emph{and} in the setting where we only consider finite models.   
%In each of these cases, the complexity is related to the complexity of the satisfiability problem for the respective logic. 
%However, for the logic of tuple-generating dependencies (TGDs) the situation is different: 

Regarding question number two, the picture is similar: under fairly weak assumptions on the logic under consideration, one can reduce the satisfiability problem for the logic to the question whether the class of models is closed under homomorphisms. 

For question three it is important to note that already for very basic first-order sentences $\phi$, the homomorphism closure $\mathcal C$ of the model class of $\phi$ is not expressible in first-order logic, and the question whether ${\mathcal C}$ is expressible in some logic with a decidable model checking problem is undecidable (Theorem~\ref{thm:excharhom}; again, the same result holds if we consider finite models only). On the other hand, we have positive results if $\phi$ has quantifier prefix $\exists^* \forall^*$ and for the trigarded and the two-variable fragments of first-order logic.

Concerning question number four,
note that the homomorphism preservation theorem provides a normal form for first-order logic, namely the existential positive fragment; and that Rossmann's theorem proves that the same normal form can be used if we consider finite models only. 
Note that computing the normal form can be quite costly: there is a potentially non-elementary blow-up for the length of a shortest equivalent existential positive formula (Theorem 6.1 in~\cite{Rossman08}). 
For finite models, there is even a non-elementary blow-up in the smallest possible quantifier-rank of an equivalent existential positive formula~\cite{Rossman08}. 
We prove that second-order logic has a normal form for sentences whose models are closed under homomorphisms, too. 
%we identity second-order sentences whose model classes are always closed under homomorphisms, and such that every second-order sentence whose model class is closed under homomorphisms is equivalent to a sentence in normal form. 
In our case, however, the normal form can be computed from the given second-order sentence in polynomial time. The statement also holds for the variant where we consider finite models only. 
An important preservation theorem from model theory is the
\emph{homomorphism preservation theorem} which asserts that a first-order sentence $\phi$ is equivalent to an existential positive sentence if and only if the class of all models of $\phi$ is preserved by homomorphisms. Existential positive sentences are studied in theoretical computer science and in particular in database theory, where they are called \emph{unions of conjunctive queries} and belong to some of the most frequently encountered database queries in practice. Classes of finite structures that are closed under homomorphisms also appear naturally in theoretical computer science; for example the complement of a constraint satisfaction problem, viewed as a class of finite structures, is closed under homomorphisms. 

Rossmann showed that that the homomorphism preservation theorem also holds if we consider homomorphisms between \emph{finite} models only. The homomorphism preservation theorem also extends to some more expressive logics: for example, Feder and Vardi (2001) proved that a Datalog$(\neg)$ program,
i.e., a Datalog program where additionally atomic negation is allowed, is equivalent to a Datalog program if and only if the class of structures defined by the program is preserved by homomorphisms; in this case it is easy to see by a compactness argument that preservation under homomorphisms for all models and for all finite models is equivalent. 


Here we will be investigate the following four types of questions:
\begin{itemize}
\item Given a sentence $\phi$ from some logic and a finite structure $\mathfrak{A}$, 
decide whether $\mathfrak{A}$ belongs the the closure of the models of $\phi$ under homomorphism. 
How difficult is this problem computationally? 
We are interested in the combined complexity (where both $\mathfrak{A}$ and $\phi$ are given) 
and in the complexity where $\mathfrak{A}$ is given and $\phi$ is fixed. 
\item Given a sentence $\phi$ from some logic, decide whether the class of models of $\phi$ is closed under homomorphisms. How difficult is this problem computationally? 
\item Given a sentence $\phi$ from some logic, 
can we compute a sentence $\psi$ (either from the same logic or from a different logic) such that
the model class of $\psi$ is precisely the homomorphism closure of the model class of $\phi$? 
\item For which logics 
is there a \emph{`syntactic normal form'} such that a sentence from that logic is equivalent to a sentence in normal form if and only if the model class is closed under homomorphisms? Of course the normal form should be effectively decidable (preferably even in polynomial time). 
\end{itemize}

If the satisfiability problem for the logic under consideration is undecidable, as for example for first-order logic, we obtain that the computational problem from question one is undecidable, too. 
However, we show that the problem is decidable in 2ExpTime for the guarded negation fragment of first-order logic, and in fact complete for this complexity class. 
We also prove decidability and complexity completeness results for the triguarded fragment, the two-variable fragment, and various quantifier prefix classes of first-order logic (Theorem~\ref{thm:first-main}). Each of the results holds both in the setting where we consider arbitrary models \emph{and} in the setting where we only consider finite models.   
%In each of these cases, the complexity is related to the complexity of the satisfiability problem for the respective logic. 
%However, for the logic of tuple-generating dependencies (TGDs) the situation is different: 

Regarding question number two, the picture is similar: under fairly weak assumptions on the logic under consideration, one can reduce the satisfiability problem for the logic to the question whether the class of models is closed under homomorphisms. 

For question three it is important to note that already for very basic first-order sentences $\phi$, the homomorphism closure $\mathcal C$ of the model class of $\phi$ is not expressible in first-order logic, and the question whether ${\mathcal C}$ is expressible in some logic with a decidable model checking problem is undecidable (Theorem~\ref{thm:excharhom}; again, the same result holds if we consider finite models only). On the other hand, we have positive results if $\phi$ has quantifier prefix $\exists^* \forall^*$ and for the trigarded and the two-variable fragments of first-order logic.

Concerning question number four,
note that the homomorphism preservation theorem provides a normal form for first-order logic, namely the existential positive fragment; and that Rossmann's theorem proves that the same normal form can be used if we consider finite models only. 
Note that computing the normal form can be quite costly: there is a potentially non-elementary blow-up for the length of a shortest equivalent existential positive formula (Theorem 6.1 in~\cite{Rossman08}). 
For finite models, there is even a non-elementary blow-up in the smallest possible quantifier-rank of an equivalent existential positive formula~\cite{Rossman08}. 
We prove that second-order logic has a normal form for sentences whose models are closed under homomorphisms, too. 
%we identity second-order sentences whose model classes are always closed under homomorphisms, and such that every second-order sentence whose model class is closed under homomorphisms is equivalent to a sentence in normal form. 
In our case, however, the normal form can be computed from the given second-order sentence in polynomial time. The statement also holds for the variant where we consider finite models only. 


==> TODO.tex <==
12 pages excluding references, British English, Appendix allowed (if not encouraged), 
double-blind, however pre-publication at ArXiV is OK 

\bigskip

$\mathfrak{A} \arbhom \mathfrak{B}$ arbitrary hom

$\mathfrak{A} \injhom \mathfrak{B}$ injective hom

$\mathfrak{A} \surhom \mathfrak{B}$ surjective hom

$\mathfrak{A} \str{\arbhom} \mathfrak{B}$ strong hom

$\mathfrak{A} \embed \mathfrak{B}$ embedding (injective + strong)

$\mathfrak{A} \sshom \mathfrak{B}$ strong surjective hom

$\mathfrak{A} \mmhom \mathfrak{B}$ monomerge



$\mathcal{C}^\cl{\arbhom} $

$\mathcal{C}^\cl{\injhom} $

$\mathcal{C}^\cl{\surhom} $

$\mathcal{C}^\cl{\str{\arbhom}} $

$\mathcal{C}^\cl{\str{\injhom}} $

$\mathcal{C}^\cl{\sshom} $


\TODO

\begin{itemize}
\item
Introduce the following notation: 
\begin{itemize}
\item $\mathrm{const}(\tau)$ (maybe also $\mathrm{rel}(\tau)$)
\item $ar(P)$ (maybe we should change it to $\mathrm{ar}(P)$) \textbf{DONE}
\end{itemize}
\item
Change 
\begin{itemize}
	\item $(.)_\mathrm{fin}$ to $(.)_{<\omega}$ \textbf{DONE}
	\item $(.)_\mathrm{ctl}$ to $(.)_{\leq\omega}$ \textbf{DONE}
\end{itemize}
\item
Read up on and succinctly present homomorphism preservation theorems in the infinite and the finite. Give enough details on the properties of the \EpFO formula obtained (in particular: quantifier rank). Place: prelims, before or after ``Recap Descriptive Complexity''.  
\item
Find reference for or prove undecidability of deterministic margin-constrained tiling problems -- reduction from TM non-halting problem (for arbitrary tilings) and TM looping problem (for ultimately periodic tilings).
\item
Provide references for the considered fragments regarding
\begin{itemize}
\item tight complexities for satisfiability (for prefix-classes, Börger, Grädel, Gurievich should provide everything needed)	
\item finite-model property -- ideally with bound on size (for prefix-classes, Börger, Grädel, Gurievich should provide everything needed)
\end{itemize}   
\item
Briefly introduce and discuss how to measure length of description for structures (distinction between $||\mathfrak{A}||$ and $|A|$ -- in particular, $||\mathfrak{A}||$ can be exponential in $|\tau| + |A|$ if arity in $\tau$ is unbounded)
\item
Cross-check claims about \textsc{LogSpace}-reducibility.
\item
Prove all (non-trivial) Lemmas, Propositions and Theorems to a sufficient level of detail. ;-)
\end{itemize}



\textbf{Up for Discussion.}

\begin{itemize}
\item
Is $\homcl{\mathcal{C}}$ good notation or should we use something else? In any case, it should go well when nested with $\getmodels{\cdot}$, so another pair of parentheses (like $\llparenthesis\mathcal{C}\rrparenthesis$) is probably not a good idea. An overline $\overline{\mathcal{C}}$ might work (a nice way to indicate closures in general) but may cause trouble with vertical line spacing, see: $\overline{\getmodels{\Phi}}$. And we always need a ``finite version''.
This would lead to something like ${\overline{\getfinmodels{\Phi}}}^\mathrm{fin}$ or rather ${\overline{\getmodels{\Phi}_{<\omega}}}^{<\omega}$
or -- when fiddling a bit with the scaling -- we'd get ${\overline{\getmodels{\Phi}_{\scaleobj{0.6}{\!<}\scaleobj{0.8}{\omega}}}}^{\scaleobj{0.6}{<}\scaleobj{0.8}{\omega}}$
  

\item
Use a specific font (typewriter?) for signature elements (relations and constants).
I think this is useful to keep track of what is going on. It just becomes a bit delicate if we a posteriori quantify over ``constants'' (turning them into variables).
\item
Put all complexities in small caps (like \textsc{NExpTime}, etc)? I am used to do this. 

\item
Different sign for implication to distinguish it from mappings? $\Rightarrow$ instead of $\to$?
Then it might clash with metalogical notation...
\item When talking about the ``normal form'' for homclosed formulae, we could investigate computational properties of a mapping $\Logic \to \Logic$ which turns every sentence into normal form but is equivalent only if the original formula was already homclosed. 
What's the complexity of the computation? What is the upper bound on the size of the created formula? This would emphasize the good properties of our $\SO$ normal form (can be computed in polytime and result is of polynomial size), but we would need to dig into the other cases... 


\end{itemize}



\neutral

==> characterization.tex <==
\section{Characterizing Homomorphism Closures Logically}\label{sec:CharHomCl}

\bigskip

\probbox{
	\textbf{Problem:} $\mathrm{CharHomCl}_{\mathrm{(fin)}}$\\
	\textbf{Input:} $\tau$, sentences $\Phi$ and $\Psi$ over $\tau$.\\
	\textbf{Output:} Yes, if $\getffinmodels{\Psi} = \homclffin{\getffinmodels{\Phi}}$, no otherwise.  
}

\bigskip

\begin{proposition}\label{prop:SatToHomCl}
	$\mathrm{HomClosed}_\mathrm{(fin)}$ can be \textsc{LogSpace}-reduced to $\mathrm{CharHomCl}_\mathrm{(fin)}$.	
\end{proposition}

\begin{proof} Pick $\Phi = \Psi$. \end{proof}

Thus, $\mathrm{CharHomCl}_\mathrm{(fin)}$ is undecidable whenever $\mathrm{HomClosed}_\mathrm{(fin)}$ is.



\Thomas 

Plan for suitable decidable fragments of FOL:

1. Check $\Phi \models \Psi$. Easy if $\Phi \wedge \neg\Psi$ is guaranteed to be in the same (or another) satisfiability-decidable fragment. Complexity: co-class of the corresponding satisfiability problem. 

2. Check $\mathrm{HomClosed}$ of $\Psi$. We know how to do this (last section). Again: complexity is co-class of the corresponding satisfiability problem.


3. Check that every model of $\Psi$ has a model of $\Phi$ as ``homomorphic origin''
Trick: given that $\Psi$'s models are homomorphism-closed we know that there is an equivalent positive existential formula with quantifier rank not higher than $\Psi$'s.
This can be converted into a UCQ where every disjunct is a CQ using only linearly many variables in the size of $\Psi$. That means, the set of models of $\Psi$ can be described as the finite union $\bigcup_{\mathfrak{A} \in \mathcal{A}} \homcl{\{\mathfrak{A}\}}$ of the element-wise homomorphism closures of a set of $\tau$-structures with domain size linearly bounded by $\Psi$ (and thus has an exponentially bounded description, thus there are at most doubly exponentially many different such structures). Clearly, then, if one of the models $\Psi$ does not have a homomorphic "origin" among the models of  
$\Phi$, there must even be one structure $\mathfrak{A} \in \mathcal{A}$ with $\mathfrak{A} \not\in \homcl{\getmodels{\Phi}}$. Hence, we can proceed as follows:
for every (of the doubly exponentially many) size-bounded $\tau$-structure $\mathfrak{A}$ check if $\mathfrak{A} \in \getmodels{\Psi}$ (``easy'', in EXPTIME since time complexity of FO model checking is $O(n^k)$ where n is the size of the structure and k the size of the formula) and, if that is the case, check $\mathfrak{A} \in \homcl{\getmodels{\Phi}}$ (in the co-class of satisfiability, here we need better bounds assuring that the results hold for any polynomial $|A|$ even if $\mathfrak{A}$ is exponential). 
We cannot test all 2Exp possibilities

%If unsatisfiability is ExpTime or higher, the exponentially many checks (on polynomial input) don't hurt and the overall check is still not harder than checking unsatisfiability in the underlying logic.

So we can test $\mathrm{CharHomCl}$ by executing 3 checks not harder than unsatisfiability.

\neutral

\begin{theorem}
	$\mathrm{CharHomCl}_{\mathrm{(fin)}}$ for
	\begin{enumerate}
		\item 
		\GNFO{} is \textsc{2ExpTime}-complete,
		\item 
		\TGF{} is \textsc{coN2ExpTime}-complete,
		\item 
		\Ct{} is \textsc{coNExpTime}-complete,
		\item 
		\AsFO{} is \textsc{coNExpTime}-complete,
		\item
		\EsFO{} is \textsc{coNExpTime}-complete,						
		\item
        \EpFO{} is \textsc{coNP}$^\textsc{NP}$-complete.						
	\end{enumerate}
\end{theorem}

\begin{proof}
For \EpFO{}, homomorphism-closedness is guaranteed to hold, therefore, the task coincides with checking equivalence of two \EpFO{} sentences, which is known to be \textsc{coNP}$^\textsc{NP}$-complete (CITE HUBIE CHEN).
For the other fragments, membership can be uniformly established via TO BE FILLED IN BY THOMAS ...
while hardness follows from the corresponding results for $\mathrm{HomClosed}_{\mathrm{(fin)}}$
in the light of Proposition~\ref{prop:SatToHomCl}.
\end{proof}


\begin{theorem}
$\mathrm{CharHomCl}_{\mathrm{(fin)}}$ is undecidable for \TGD{}.
\end{theorem}

\begin{proof}
We show that the undecidable problem of checking whether a boolean conjunctive query Q is entailed from a \TGD{} sentence $\Phi$ can be \textsc{LogSpace}-reduced to $\mathrm{CharHomCl}_{\mathrm{(fin)}}$. We define $\Phi_Q$ as $\Phi\wedge (Q \to CQ(\mathfrak{F}))$. Then $\Phi \models Q$ exactly if 	
$ \homclffin{\getffinmodels{\Phi_Q}} = \getffinmodels{CQ(\mathfrak{F})} $
%
\end{proof}


==> generic-type-approach.tex <==
We will find it useful to first ask for projective characterizations of homclosures.  

\begin{definition}
For logics $\Logic, \Logic' \subseteq \SO$, we say $\Logic'$ \emph{homcaptures} $\Logic$ if for every $\tau$ and $\Logic$ $\tau$-sentence $\Phi$ there exist some $\sigma$ and a $\Logic'$ $\tau{\uplus}\sigma$-sentence $\Psi$ such that  $\homcl{\getmodels{\Phi}} = \getmodels{\Psi}|_{\tau}$.   
\end{definition}

Note that whenever $\Logic'$ \emph{homcaptures} $\Logic$, it follows that for any $\Logic$ sentence $\Phi$, we find a $\ESO(\Logic')$ sentence characterizing $\Phi$'s homclosure, where $\ESO(\Logic')$ denotes sentences led by second-order existential quantifiers followed by a $\Logic'$ sentence.   

We will next give a high-level description of a generic type-based approach which will be applicable to all mentioned logics with slight variations in the details. 

To this end, we fix a signature $\tau$ and introduce the notion of an \emph{$n$-type} as a maximally consistent set $\tp$ of literals (i.e., negated and unnegated atoms) using all constants from $\tau$ and a finite collection of variables $v_1,\ldots,v_n$ (denoted $\bold{v}$) disjoint from the variables used in the considered sentence. 
Where convenient, we identify the (necessarily finite) set $\tau$ with $\bigwedge\tau$. 
We say an $n$-type $\tp$ is \emph{realized} by an $n$-tuple $\bold{a} = (a_1,\ldots,a_n) \in A^n$ of domain elements of a $\tau$-structure $\mathfrak{A}$, if $(\mathfrak{A},\{v_i \mapsto a_i\}) \models \tp$. We say $\tp$ is \emph{realized} ($k$ times) in $\mathfrak{A}$ if it is realized by ($k$ distinct) tuples of $\mathfrak{A}$. Note that every tuple $\bold{a}$ realizes one unique type, which entirely characterizes the substructure of $\mathfrak{A}$ induced by all the elements of $\bold{a}$ together with all elements denoted by constants.   
In our construction, we will make use of the fact that for several logics, many questions regarding a structure can be answered, if one knows what types of a certain kind are realized in that structure. On a generic level, we assume there is a function that, given a $\tau$-sentence $\Phi$ yields a finite set $\mathcal{E}$ of \emph{eligible types} (with possibly varying $n$), which are sufficient for our purposes. Then, given a $\tau$-structure $\mathfrak{A}$, we let its \emph{type summary} $\mathcal{E}(\mathfrak{A})$ denote the pair $(\mathcal{E}_\text{+},\mathcal{E}_!)$ where $\mathcal{E}_\text{+}$ ($\mathcal{E}_!$) consists of those types from $\mathcal{E}$ realized (exactly once) in $\mathfrak{A}$. Furthermore, the \emph{model summary} $\getsummary{\Phi}$ of a sentence $\Phi$ is defined by $\{\mathcal{E}(\mathfrak{A}) \mid \mathfrak{A} \in \getmodels{\Phi}\}$, which is a finite set by assumption. 

We will extend our signature by a set $\sigma$ of \emph{type predicates}, containing an $n$-ary predicate symbol $\Tp_\tp$ for every eligible $n$-type $\tp \in \mathcal{E}$.
Given a $\tau$-structure $\mathfrak{A}$ and a set $\mathcal{E}$ of eligible types over $\tau$, the \emph{$\mathcal{E}$-adornment} of $\mathfrak{A}$, denoted $\mathfrak{A}\cdot\mathcal{E}$ is the $\tau\uplus\sigma$-structure expanding $\mathfrak{A}$ such that
$\Tp_\tp^{\mathfrak{A}\cdot\mathcal{E}} = \{ \bold{a} \mid \bold{a} \text{ realizes } \tp \text{ in } \mathfrak{A} \}$. In a way, $\mathcal{E}$-adornments materialize the information regarding relevant types in a model. While this information is obviously redundant in the model itself, we will make good use of it when characterizing a model's homomorphic targets.

Given a $\tau$-sentence $\Phi$ (which we presume to be in some normal form with bounded quantifier alternation), we will construct a $\tau\uplus\sigma$-sentence $\Psi$ that (projectively) identifies those $\mathfrak{B}$ into which some model $\mathfrak{A}$ of $\Phi$ has a homomorphism $h:\mathfrak{A} \arbhom \mathfrak{B}$, using the following idea: assuming such an $h$ exists, then it will also serve as homomorphism from $\mathfrak{A}\cdot\mathcal{E}$ to $\mathfrak{B}'$, where $\mathfrak{B}'$ expands $\mathfrak{B}$ by letting $\Tp_\tp^{\mathfrak{B}'} = \{ (h(a_1),\ldots,h(a_n)) \mid (a_1,\ldots,a_n) \in \Tp_\tp^{\mathfrak{A}\cdot\mathcal{E}} \}$, that is, where all type information materialized in $\mathfrak{A}$ is transferred to $\mathfrak{B}$ along $h$. In fact, $\Psi$ is then built in a way that its models are precisely such $\mathfrak{B}'$.

One integral part of $\Psi$ is to ensure that the way types are mapped to $\mathfrak{B}$ is compatible with the homomorphism condition:
$$\bigwedge_{\tp \in \mathcal{E}} \forall \bold{v}.\big( \Tp_\tp(\bold{v}) \impl \bigwedge \{\alpha \in \tp \mid \alpha \text{ positive literal}\} \big)$$
Moreover, we require that the collection of ``transferred type atoms'' found in $\mathfrak{B}'$ corresponds to the type summary of some model. To this end we include in $\Psi$ a case distinction 
$\bigvee_{(\mathcal{E}_\text{+},\mathcal{E}_!)\in \getsummary{\Phi}} \Psi_{(\mathcal{E}_\text{+},\mathcal{E}_!)}$, where each $\Psi_{(\mathcal{E}_\text{+},\mathcal{E}_!)}$ details existence and relationships between the mapped types. Some of the conditions specified in $\Psi_{(\mathcal{E}_\text{+},\mathcal{E}_!)}$ are generically derived from $(\mathcal{E}_\text{+},\mathcal{E}_!)$, others are obtained by translating constraints from $\Phi$ into ``type language'', expressed by type atoms.
By construction, the sentence $\Psi$ thus obtained holds in some type-adorned structure $\mathfrak{A}\cdot\mathcal{E}$ precisely if $\mathfrak{A} \in \getmodels{\Phi}$ and its satisfaction is preserved under ``type-faithful'' homomorphisms  $h:\mathfrak{A}\cdot\mathcal{E} \arbhom \mathfrak{B}'$ as described above, thus ensuring $\homcl{\getmodels{\Phi}} \subseteq \getmodels{\Psi}|_{\tau}$.
The other direction $\homcl{\getmodels{\Phi}} \supseteq \getmodels{\Psi}|_{\tau}$ is shown by taking a model $\mathfrak{B}'$ and ``unfolding'' or  ``unraveling'' it such that, in the resulting structure, the diverse $\Tp_\tp$ instances do not provide contradicting information about the $\tau$-connections between their arguments.


Instantiating the described strategy, we obtain the following theorem.

\begin{theorem}
\begin{enumerate}
\item $\FOte$ homcaptures itself.
\item $\TGF$ homcaptures itself and $\EAAE$.
\item $\GFO$ homcaptures itself and $\GNFO$.
\end{enumerate}
\end{theorem}

In view of our earlier discussion, this means that all these logics admit homclosure characterization in $\ESO$.

\begin{corollary}
	For any fixed \FOte, \TGF{}, \EAAE, \GFO{} or \GNFO{} sentence $\Phi$, checking $\mathfrak{A} \in \homcl{\getmodels{\Phi}}$ 
	%for finite structures $\mathfrak{A}$ 
	is in \textsc{NP}.   
\end{corollary}
 
We next complement these $\textsc{NP}$-membership results by providing matching lower bounds even for much weaker logics.

\newcommand{\narrowimp}{ \!\! & {\!\!\!\!\!\!{\impl}\!\!\!\!\!\!} &  \!\! }
\newcommand{\narrowwedge}{\,{\wedge}\,}
\newcommand{\narrowvee}{\,{\vee}\,}

\begin{definition}[restate=phithreesat, name=]\label{def: 3SAT}
	We let $\Phi_\mathrm{3SAT}$ be the sentence containing the conjunction of the following sentences (leading universal quantifier omitted):
	\begin{eqnarray}
		& & \!\!  \exists x. \sig{First}(x) \\
		%
		\sig{First}(x)
		\narrowimp
		\sig{CLst}(x)\ \ \ \ \ \\
		%
		\sig{CLst}(x)
		\narrowimp
		\exists y. \sig{Next}(x,y) \narrowwedge \big(\sig{CLst}(y) \narrowvee \sig{Nil}(y)\big)\ \ \ \ \ \\
		%	
		\sig{CLst}(x) 
		\narrowimp 
		\exists y. \sig{Lit}(x,y)  \wedge \sig{Sel}(y)
		\\
		%
		\sig{Sel}(x) \narrowwedge \sig{Sel}(y) 
		\narrowimp 
		\sig{Cmp}(x,y).
	\end{eqnarray}
	For a given instance of 3SAT $\mathcal{S} = \{C_1, \ldots, C_n\}$ consisting of $n$ clauses each containing 3 literals over propositional variables $p_1,\ldots,p_m$, define the structure $\mathfrak{A}_{\mathcal{S}}$ by letting
	%
	\begin{eqnarray}
		A_\mathcal{S} & {\!\!\!\!=\!\!\!\!} & \{a_i \mid 1\leq i\leq n+1\} \cup \{b_i, b'_i \mid 1\leq i\leq m\}\ \ \ \ \ \\
		\sig{First}^{\mathfrak{A}_{\mathcal{S}}} & {\!\!\!\!=\!\!\!\!} & \{a_1\}\\
		\sig{CLst}^{\mathfrak{A}_{\mathcal{S}}} & {\!\!\!\!=\!\!\!\!} & \{a_i \mid 1\leq i\leq n\}\\
		\sig{Nil}^{\mathfrak{A}_{\mathcal{S}}} & {\!\!\!\!=\!\!\!\!} & \{a_{n+1}\}\\
		\sig{Next}^{\mathfrak{A}_{\mathcal{S}}} & {\!\!\!\!=\!\!\!\!} & \{(a_i,a_{i+1}) \mid 1\leq i\leq n\}\\
		\sig{Lit}^{\mathfrak{A}_{\mathcal{S}}} & {\!\!\!\!=\!\!\!\!} & \{(a_i,b_j) \mid p_j \in C_i\} \cup \{(a_i,b'_j) \mid \neg p_j \in C_i\}\\
		\sig{Sel}^{\mathfrak{A}_{\mathcal{S}}} & {\!\!\!\!=\!\!\!\!} & \{b_i, b'_i \mid 1\leq i\leq m\}\\
		\sig{Cmp}^{\mathfrak{A}_{\mathcal{S}}} & {\!\!\!\!=\!\!\!\!} & \{(b_i,b_j),(b'_i,b'_j),(b_i,b'_k),(b'_i,b_k) \mid i\not= k\}
	\end{eqnarray}
\end{definition}
%
Obviously, $\Phi_\mathrm{3SAT}$ is contained in constant-free, equality-free $\FOt$ (and therefore in $\FOte$ and \TGF). Also, it can be 
rewritten into constant-free, equality-free $\Al\Al\Ex\Ex\FO$ (and therefore into 
$\EAAE$). Also, the 3SAT instance $\bigwedge_{\{\ell,\ell',\ell''\}\in \mathcal{S}} \ell {\vee} \ell' {\vee} \ell''$ is satisfiable exactly if $\mathfrak{A}_\mathcal{S} \in \homcl{\getffinmodels{\Phi_\mathrm{3SAT}}}$. Hence we obtain the following statement, providing matching lower bounds.

\begin{proposition}[restate=NPhardFOprop, name=]
Checking homclosure membership is \textsc{NP}-hard for constant-free, equality-free $\FOt$ and $\Al\Al\Ex\Ex\FO$ with predicate arity $\leq 2$.
\end{proposition}

Note that this settles the case of the data complexity of homclosure membership for any logic between $\FOt$ or $\Al\Al\Ex\Ex\FO$ on the lower and  $\FOte$, $\TGF{}$, or $\EAAE$ on the upper end, showing that one cannot hope for characterizability in a logic with lower complexity. It does not provide a lower bound for $\GFO$ or $\GNFO$, though. 

